On Differentially Private 3D Medical Image Synthesis with Controllable Latent Diffusion Models

Generally, the small size of public medical imaging datasets coupled with stringent privacy concerns, hampers the advancement of data-hungry deep learning models in medical imaging. This study addresses these challenges for 3D cardiac MRI images in the short-axis view. We propose Latent Diffusion Models that generate synthetic images conditioned on medical attributes, while ensuring patient privacy through differentially private model training. To our knowledge, this is the first work to apply and quantify differential privacy in 3D medical image generation. We pre-train our models on public data and finetune them with differential privacy on the UK Biobank dataset. Our experiments reveal that pre-training significantly improves model performance, achieving a Fr\'echet Inception Distance (FID) of 26.77 at $\epsilon=10$, compared to 92.52 for models without pre-training. Additionally, we explore the trade-off between privacy constraints and image quality, investigating how tighter privacy budgets affect output controllability and may lead to degraded performance. Our results demonstrate that proper consideration during training with differential privacy can substantially improve the quality of synthetic cardiac MRI images, but there are still notable challenges in achieving consistent medical realism.

==> sections/02_Background.tex <==
% !TeX root = ../main.tex

%\section{Background}



==> sections/Old.tex <==




\subsection{Old}
"The measurement of ventricular volumes, mass, and systolic func- tion allows identification and grading of pathologies, prognostic assessment, and the monitoring of changes under therapy. For example, myocardial wall thickness in hypertrophic cardiomy- opathy (HCM) and the ejection fraction (EF) in heart failure act as key parameters for defibrillator or resynchronization therapy." \cite{Seraphim2020QuantitativeMRI}


Segmentation model metrics used for ejection fraction calculation:
  validation accuracy:          98.81\%
  validation Dice LV:           0.916444
  validation Dice Myo:          0.891805
  validation Dice RV:           0.958841





1. best config for high quality images with this:
ESED score, correlation with LVEF 
\begin{table}[ht]
\centering
\begin{tabular}{lcccc}
\hline
Model & \multicolumn{2}{c}{2x compression} & \multicolumn{2}{c}{4x compression} \\ \cline{2-5} 
 & FID & MS-SSIM & FID & MS-SSIM \\ \hline
KL-VAE & X.XX & Y.YY & A.AA & B.BB \\
VQ-VAE & C.CC & D.DD & E.EE & F.FF \\ \hline
\end{tabular}
\caption{Comparison of KL-VAE and VQ-VAE at 2x and 4x compression rates}
\label{tab:diffusion_models_metrics}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{lcccccccc}
\hline
Model & \multicolumn{4}{c}{2x compression} & \multicolumn{4}{c}{4x compression} \\ \cline{2-9} 
 & FID & MS-SSIM & ES/ED Acc. & EF Corr. & FID & MS-SSIM & ES/ED Acc. & EF Corr. \\ \hline
KL-VAE & X.XX & Y.YY & G.GG & H.HH & A.AA & B.BB & I.II & J.JJ \\
VQ-VAE & C.CC & D.DD & K.KK & L.LL & E.EE & F.FF & M.MM & N.NN \\ \hline
\end{tabular}
\caption{Extended comparison of KL-VAE and VQ-VAE at 2x and 4x compression rates with added performance metrics}
\label{tab:diffusion_models_metrics_extended}
\end{table}



Three privacy categories low, medium, high
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
\hline
Model & \multicolumn{2}{c}{128 Channels} \\ \cline{2-3} 
 & FID & MS-SSIM \\ \hline
With Differential Privacy & P.PP & Q.QQ \\
Without Differential Privacy & R.RR & S.SS \\ \hline
\end{tabular}
\caption{Comparison of models with and without differential privacy for the 128 channels case}
\label{tab:privacy_diff_channels}
\end{table}



\begin{table}[ht]
\centering
\begin{tabular}{lcccccc}
\hline
Model & \multicolumn{2}{c}{64 channels} & \multicolumn{2}{c}{128 channels} & \multicolumn{2}{c}{192 channels} \\ \cline{2-7} 
 & FID & MS-SSIM & FID & MS-SSIM & FID Score & MS-SSIM \\ \hline
KL-VAE & P.PP & Q.QQ & R.RR & S.SS & T.TT & U.UU \\
VQ-VAE & V.VV & W.WW & X.XX & Y.YY & Z.ZZ & A1.A1 \\ \hline
\end{tabular}
\caption{Comparison of different model sizes}
\label{tab:model_sizes_metrics}
\end{table}




\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{img/DPDummyComparison.png}
    \caption{DP Dummy Comparison}
    \label{fig:enter-label}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{img/ConditioningDummyComparison.png}
    \caption{Conditioning Dummy Comparison}
    \label{fig:enter-label}
\end{figure}
